Defending against Insertion-based Textual Backdoor Attacks via Attribution

Textual backdoor attack, as a novel attack model, has been shown to be effective in adding a backdoor to the model during training. Defending against such backdoor attacks has become urgent and important. In this paper, we propose AttDef, an efficient attribution-based pipeline to defend against two insertion-based poisoning attacks, BadNL and InSent. Specifically, we regard the tokens with larger attribution scores as potential triggers since larger attribution words contribute more to the false prediction results and therefore are more likely to be poison triggers. Additionally, we further utilize an external pre-trained language model to distinguish whether input is poisoned or not. We show that our proposed method can generalize sufficiently well in two common attack scenarios (poisoning training data and testing data), which consistently improves previous methods. For instance, AttDef can successfully mitigate both attacks with an average accuracy of 79.97% (56.59% up) and 48.34% (3.99% up) under pre-training and post-training attack defense respectively, achieving the new state-of-the-art performance on prediction recovery over four benchmark datasets.

==> figures/threshold_BERT.tex <==
% \begin{figure}[!th]
% \centering
% \includegraphics[width=\linewidth]{figures/threshold_ONION_offenseval.png}
% \includegraphics[width=\linewidth]{figures/threshold_BF_offenseval.png}
% \caption{The relationship between $\bigtriangledown$ASR (in red) and $\bigtriangledown$CACC (in blue) and attention threshold when against 4 post-training attacks. \emph{BadNL} backdoor attacks variants denotes as $BL$ with frequency subscript, \emph{InSent} backdoor attack denotes as \emph{InS}}
% \label{fig:threshold}
% \end{figure}












\begin{figure*}
    \centering % <-- added
\begin{subfigure}{0.4\textwidth}
  \includegraphics[width=\linewidth]{figures/threshold_ONION_offenseval.png}
  \caption{\method against post-training attack }
  \label{Attention_clean}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.4\textwidth}
  \includegraphics[width=\linewidth]{figures/threshold_BF_offenseval.png}
  \caption{\method against pre-training attack }
  \label{Attention_poison}
\end{subfigure}\hfil % <-- added
\caption{The relationship of $\Delta$ASR (in red) and $\Delta$CACC (in blue) and attention threshold against post-training attack(left) and post-training attack (right). }
\label{fig:threshold}
\end{figure*}


% \begin{figure}
%     \centering % <-- added
% \begin{subfigure}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{figures/threshold_ONION_offenseval.png}
%   % \caption{\method against post-training attack }
%   \label{Attention_clean}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.24\textwidth}
%   \includegraphics[width=\linewidth]{figures/threshold_BF_offenseval.png}
%   \caption{\method against pre-training attack }
%   \label{Attention_poison}
% \end{subfigure}\hfil % <-- added
% \caption{The relationship between $\bigtriangledown$ASR (in red) and $\bigtriangledown$CACC (in blue) and attention threshold when against 4 post-training attacks. $BL$ denotes \emph{BadNL} backdoor attacks variants, \emph{InS} denotes \emph{InSent} backdoor attack}
% \label{fig:threshold}
% \end{figure}

==> tables/Result_ONION_CNN_table_4.tex <==
\begin{table*}[tb]
\centering
\small
\begin{tabular}{|l|rr|rr|rr|}\hline  

&\multicolumn{2}{|c|}{\textbf{Poisoned Model}}& \multicolumn{4}{c|}{\textbf{Defense Result}} \\ \hline 

&\multicolumn{2}{|c}{\textbf{}}
&\multicolumn{2}{|c}{\textbf{BFClass}}
&\multicolumn{2}{|c|}{\textbf{Electra+\method}}\\\hline

 \textbf{Attacks} &\textbf{CACC} & \textbf{ASR}& \textbf{$\bigtriangledown$ASR} & \textbf{$\bigtriangledown$CACC} & \textbf{$\bigtriangledown$ASR} & \textbf{$\bigtriangledown$CACC}\\ \hline

\emph{BadNL}$_l$ & 75.79  & 97.72 &  14.1  &  0.81  & 80.89 & 10.49\\ 
\emph{BadNL}$_m$ & 75.31 &  96.71  &  28.09 &  -0.04 &  76.43 & 10.55 \\ 
\emph{BadNL}$_h$& 72.49 &  67.21 &  -3.05  & 1.48  &   29.74 & 8.99 \\ 
\emph{InSent}  &  75.6  & 100   &  0  &  1.3  &  69.63 & 10.5  \\ 
\emph{Avg}     & 74.8  & 90.41 &  9.79 &  0.89 &  64.17 & 10.13\\ \hline

\end{tabular}
\caption{\label{tab:result_CNN_ONION} Comparison of \method with ONION on CNN attack success rate and clean accuracy against two data poisoning attacks on two different datasets.}

\end{table*}

==> tables/Result_ONION_Substituion.tex <==

\begin{table}[h]
\centering
\small
% \begin{tabular}{|l|rr|rr|rr|}\hline  
\begin{tabular}{|l|cc|cc|}\hline  

&\multicolumn{2}{|c}{\textbf{Poisoned Model}}
&\multicolumn{2}{|c|}{\textbf{\method}}\\\hline

 % \textbf{Attacks} &\textbf{CACC} & \textbf{ASR}& \textbf{$\bigtriangledown$ASR} & \textbf{$\bigtriangledown$CACC} & \textbf{$\bigtriangledown$ASR} & \textbf{$\bigtriangledown$CACC}\\ \hline
 \textbf{Attack}& \textbf{ASR} & \textbf{CACC} & \textbf{$\Delta$ASR} & \textbf{$\Delta$CACC}\\ \hline

\emph{Benign}&   - &  91.84  &  -  & 1.68 \\
\emph{LWS}  & 98.25  & 88.72   &  2.69 & 3.4 \\\hline

\end{tabular}
\caption{}
\label{tab:Result_Substitution}
\end{table}

==> tables/compared_with_RAP.tex <==
\begin{table}
\centering
\begin{tabular}{l|ccc|c}
\hline \textbf{Task} & \textbf{target class} & \textbf{} & \textbf{Test} & \textbf{Avg Len}\\ \hline
SST-2 & 6.9K &  873 & 1.8K & 19.3 \\
OLID & 11.9K &  1.3K & 859 & 23.9 \\
AGNews & 110K &  10K & 7.6K & 38.4\\
IMDB & 25K &  8.3K & 16.8K & 231.1\\\hline
\end{tabular}
\caption{\label{dataset} Overview of datasets used in this study with short-length (SST-2), mediam-length (OLID and AGNews) and document-length (IMDB)}
\end{table}
